Privacy-Preserving Platform for Transactive Energy Systems

Transactive energy systems (TES) are emerging as a transformative solution for the problems faced by distribution system operators due to an increase in the use of distributed energy resources and a rapid acceleration in renewable energy generation. These, on one hand, pose a decentralized power system controls problem, requiring strategic microgrid control to maintain stability for the community and for the utility. On the other hand, they require robust financial markets operating on distributed software platforms that preserve privacy. In this paper, we describe the implementation of a novel, blockchain-based transactive energy system. We outline the key requirements and motivation of this platform, describe the lessons learned, and provide a description of key architectural components of this system.

==> MyPreamble.tex <==
% PACKAGES:
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{amsthm}  % used to make theoremstyles not italic
\usepackage{psfrag}
\usepackage{textcomp}
\usepackage{amsthm}
\usepackage{setspace}
\usepackage{hyperref}
\usepackage{wasysym}
\usepackage{latexsym}
\usepackage{xfrac}
\usepackage{relsize}
\usepackage{pmat}
\usepackage{url}
\usepackage{comment}
\usepackage{pdfsync}

\usepackage[cal=cm]{mathalfa} %this is to get the proper caligraphic font \mathcal and \mathbb (google mathalfa for documentation on how to use)




%\usepackage[margin=1in]{geometry}



%\usepackage[latin1]{inputenc}

% MY COMMANDS
\newcommand{\dt}{\frac{d}{dt}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\tpd}[2]{\tfrac{\partial #1}{\partial #2}}
\newcommand{\aHalf}{\frac{1}{2}}
\newcommand{\aFourth}{\frac{1}{4}}
\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator*{\argmin}{arg\;min}
\DeclareMathOperator{\co}{co}
\newcommand{\del}{\nabla}
\newcommand{\vs}{V_{\Sigma}}
\newcommand{\vo}{V_{\mathcal{O}}}
\newcommand{\dvo}{\Delta V_{\mathcal{O}}}
\newcommand{\dv}{\Delta v^k}
\newcommand{\ol}{\Omega_{\mathit{l}}}
\newcommand{\dvoh}{\Delta V_{\hat{\mathcal{O}}}}
\newcommand{\oh}{\hat{\mathcal{O}}}
\newcommand{\omo}{\Omega_{\mathcal{O}}}
\newcommand{\oms}{\Omega_{\Sigma}}
\newcommand{\omz}{\Omega_z}
\newcommand{\dis}{|y-y^*|}
\newcommand{\dist}{\|y-\mathbf{P}_{X^*}(y)\|}
\newcommand{\1}{\mathbf{1}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\delxi}{\del_{\!\!x_i}}
\newcommand{\sumiv}{\sum_{i\in\mathcal{V}}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Iota}[1]{\mathlarger{\iota}_{#1}\!}
\newcommand{\lst}[1]{\langle {#1} \rangle\!}
\newcommand{\lsti}[2]{\langle {#1} \rangle\!_{{#2}}^{-1}}
\newcommand{\eg}{{e.g., }}
\newcommand{\ie}{{\it i.e., }}
\newcommand{\st}{\:|\:}
\newcommand{\Pxi}{\mathbf{P}_{X_i}}
\newcommand{\PXi}{\mathbf{P}_{\Xi}}
\newcommand{\Pxhat}{\mathbf{P}_{\hat{X}}}
\newcommand{\Pxst}{\mathbf{P}_{X^*}}
\newcommand{\Pgo}{\mathbf{P}_{\Gamma_0}}
\newcommand{\Pc}{\mathbf{P}_{S}}
\newcommand{\Pa}{\mathbf{P}_{\!\!\mathcal{A}}}
\newcommand{\AIn}{(A\otimes I_n)}
\newcommand{\MIn}{(M\otimes I_n)}
\newcommand{\onetin}{(\mathbf{1}_N^T\otimes I_n)}
\newcommand{\Vo}{V_{\mathcal{O}}}
\newcommand{\Vc}{V_{\mathcal{C}}}
\newcommand{\Ap}{\mathcal{A}^{\bot}}
\newcommand{\Bxst}[1]{\bar{B}_{#1}(X^*)}
\newcommand{\Bgo}[1]{\bar{B}_{#1}(\Gamma_0)}
\newcommand{\Bsqy}{ \bar{B}^n_{\!\!\!\!\sqrt{\sfrac{\delta}{2}}}(X^*)}
\newcommand{\Bsqz}{ \bar{B}^{Nn}_{\!\!\!\sqrt{\sfrac{\delta}{2}}}(\{\0\})}


% MATH OPERATORS
%\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\dg}{diag}
\DeclareMathOperator{\setspan}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\tr}{tr}

% THEOREM STYLES
 \theoremstyle{remark} %makes defs etc not italic. Must use with amsthm package
\newtheorem{assump}{A\!\!}[section]
\newenvironment{assumpPrime}[1]
  {\renewcommand{\theassump}{\ref{#1}$'$}%
   \addtocounter{assump}{-1}%
   \begin{assump}}
  {\end{assump}}
\newtheorem{lem}{Lemma}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{ex}{Example}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{alg}{Algorithm}[section]
\newtheorem{constr}{Construction}[section]


